Detecting Heavy Hitters in the Data-plane

The ability to detect, in real-time, heavy hitters is beneficial to many network applications, such as DoS and anomaly detection. Through programmable languages as P4, heavy hitter detection can be implemented directly in the data-plane, allowing custom actions to be applied to packets as they are processed at a network node. This enables networks to immediately respond to changes in network traffic in the data-plane itself and allows for different QoS profiles for heavy hitter and non-heavy hitter traffic. Current interval-based methods that flush the whole counting structure are not well-suited for programmable hardware (the data-plane), because they either require more resources than available in that hardware, they do not provide good accuracy, or require too many actions from the control-plane. A sliding window approach that maintains accuracy over time would solve these issues. However, to the best of our knowledge, the concept of sliding windows in programmable hardware has not been studied yet. In this paper, we develop streaming approaches to detect heavy hitters in the data-plane. We consider the problems of (1) adopting a sliding window and (2) identifying heavy hitters separately and propose multiple memory- and processing-efficient solutions for each of them. These solutions are suitable for P4 programmable hardware and can be combined at will to solve the streaming variant of the heavy hitter detection problem.

==> chapters/evaluationgated.tex <==
%\subsection{Memory consumption and processing time}

%\textbf{Processing time}

%\textbf{Memory.}
%Register tables, containing counters as well as the ring array (5 register arrays to store values for each of 5 tuple), are stored in the external memory (8GB available at the Netronome card) and are equal to $log(N) x width$ and $13B x N$ bytes. However, when inspecting the memory maps generated by the we noticed that the compiler generated arrays that are each $4B x N$ resulting in $20B x N$ for the ring array. 
%For larger values of N larger than $2^26$ (which corresponds to approximately last 2 sec), the ring implementation is not feasible and the corresponding firmware cannot be generated, as shown in Fig. \ref{fig:memory}.
%To achieve the same accuracy, the Gated sketch needs $\approx$ less memory. 


%\subsection{Accuracy}



\subsection{Accuracy of the Hybrid Window}

\begin{figure*}[tbh!]
\centering
\input{figures/windowEvaluation}
\caption{Comparison of the Gated sketch and the Count-Min sketch for different number of stages and widths by classifying UDP and TCP packets using 20 different CAIDA traces. Used window size 65536, the threshold 0.1\% (65 packets) and the confidence interval 95\%}\label{fig:mininet}
\end{figure*}

\subsection{Accuracy of Sequential flushing}

The probability of false positives is under 6\% and the probability of false negatives under 2\% if this scheme is used with a count-min sketch with a width of 8192, depth 3 and the heavy hitter threshold set to $0.1\% \cdot N$ for values of N between 215 and 220.  The probability of false positives, as well as false negatives decreases for higher values of N.

\subsection{Accuracy of the Hybrid window}
Initial evaluation shows that the probability of false positives is under 3.5\% and the probability of false negatives under 0.01\% if this scheme is used with a count-min sketch (with a width of 8192 and depth 1), the heavy hitter threshold set to $0.1\% \cdot N$ and N equal to $2^{15}$. By increasing the value of N (and the value of k at the same time) from $2^{15}$ to $2^{20}$ the probability of false negatives is increased but remains under 0.5\% while the probability of false positives is reduced to less than 1.3\%.

\textbf{Number of false positives.}


\textbf{Number of false negatives.} 
%The number of false negatives is low in all implementations and equal to 0 for the $th\_w=0$. In case of a high $th\_w$ the number of false negatives reduces with the increase of the width since the probability of decreasing the count for the packet that was just added is lower. 


